Memory-Constrained Semantic Segmentation for Ultra-High Resolution UAV Imagery

Amidst the swift advancements in photography and sensor technologies, high-definition cameras have become commonplace in the deployment of Unmanned Aerial Vehicles (UAVs) for diverse operational purposes. Within the domain of UAV imagery analysis, the segmentation of ultra-high resolution images emerges as a substantial and intricate challenge, especially when grappling with the constraints imposed by GPU memory-restricted computational devices. This paper delves into the intricate problem of achieving efficient and effective segmentation of ultra-high resolution UAV imagery, while operating under stringent GPU memory limitation. The strategy of existing approaches is to downscale the images to achieve computationally efficient segmentation. However, this strategy tends to overlook smaller, thinner, and curvilinear regions. To address this problem, we propose a GPU memory-efficient and effective framework for local inference without accessing the context beyond local patches. In particular, we introduce a novel spatial-guided high-resolution query module, which predicts pixel-wise segmentation results with high quality only by querying nearest latent embeddings with the guidance of high-resolution information. Additionally, we present an efficient memory-based interaction scheme to correct potential semantic bias of the underlying high-resolution information by associating cross-image contextual semantics. For evaluation of our approach, we perform comprehensive experiments over public benchmarks and achieve superior performance under both conditions of small and large GPU memory usage limitations. We will release the model and codes in the future.

==> a_intro_v1.tex <==
\section{Introduction}

Recently, with the rapid progress of photography and sensor technologies, there is a growing demand for ultra-high resolution image (i.e., 2K, 4K, or even higher resolution images) analysis due to the unique role in remote sensing and medical applications, such as urban planning, environmental assessment, and medical diagnosis. However, handling ultra-high resolution image, especially for semantic segmentation task, will cost more unaffordable computing resources.

% In order to resolve ultra-high resolution semantic segmentation, there are currently two mainstream frameworks, \ie, the cropping-segmenting-merging framework \cite{chen2019collaborative, huynh2021progressive, li2021contexts} and the shallow-deep fusion framework \cite{guo2022isdnet}, denoted as CSM and SDF for brevity, respectively. In the CSM framework, extra context beyond the local patch of ultra-high resolution image needs to be introduced to avoid degraded local segmentation caused by too narrow a view. However, it will also bring more memory and time consumption. On the other hand, the SDF framework is designed to fuse the high-resolution yet noisy semantic estimation from shallow network and the low-resolution semantic estimation from deep network, which turns out to be efficient but unavoidably introduces noise and loses details during fusion. More importantly, with the increase of input image resolution, both frameworks inevitably cost more memory.

% In order to resolve ultra-high resolution semantic segmentation, there are currently two mainstream frameworks, \ie, the cropping-segmenting-merging framework \cite{chen2019collaborative, huynh2021progressive, li2021contexts} and the end-to-end global segmentation framework \cite{guo2022isdnet}, denoted as CSM and EGS for brevity, respectively. In the CSM framework, local patch segmentation of ultra-high resolution image will reduces the need for GPU memory but consume much time. Besides, extra context beyond the local patch needs to be introduced to avoid degraded local segmentation caused by too narrow a view. This will also bring more memory and time consumption, and the context size needs to be preset according to experience. On the other hand, the latest EGS framework is designed to fuse the high-resolution yet noisy semantic estimation from shallow network and the low-resolution semantic estimation from deep network, which turns out to be efficient but unavoidably introduces noise and loses details during fusion. More importantly, with the increase of input image resolution (as shown in Fig.~\ref{fig:gpu}), most methods inevitably cost more memory. Especially in the EGS framework, memory consumption will increase rapidly.

% most of the existing models follow the three-step procedure of cropping, segmenting, and merging for local inference to reduce memory. Nevertheless, these methods introduce context outside the local image to enhance local segmentation, which costs extra memory and time. Additionally, due to slow local inference speed, a recent method ISDNet speeds up segmentation by adopting the bilateral architecture with global image context for global inference. Inevitably, as resolution increases, the memory usage for this method increases dramatically.

% To address the aforementioned limitations, we present a novel model that can be adapted to both frameworks . Specifically, our proposed model serves as the local segmentation module of CSM without introducing additional computational overhead for contexts beyond the local patch. Additionally, it can be directly used for the global inference of SDF, achieving better segmentation performance than prior art. To accomplish this, we drew inspiration from the idea of implicit neural representation (INR) \cite{} and designed an efficient spatial-guided high-resolution query module. This module enhances shallow-deep fusion in image detail inference, enabling our model to infer high-quality pixel-wise segmentation results. Our model queries the latent embeddings of the nearest spatial coordinates and the high-resolution spatial information as guidance, reducing the dependency on extra contextual information to the largest extent.
% Unlike previous feature fusion \cite{hu2022learning}, our approach guides the latent embeddings to supplement details through structurally understandable/interpretable shallow masks, which is more efficient and effective. However, the high-resolution spatial information tends to introduce semantic estimation bias during inference. To address this concern, we introduce a memory-based interaction scheme to bridge the semantic information of low-resolution features and high-resolution spatial information. This scheme implicitly introduces cross-image context for semantic-level regularization.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{iccv2023AuthorKit/figure/GPU.png}
%     \caption{The curve between input image resolution and inference memory in our model. As input image resolution increases, memory usage will increase rapidly. In the EGS framework, the memory consumption exceeds 10,000 MB when the image resolution reaches 6,000×6,000. To trade off performance and memory, our designed model in the CSM framework is comparable to that in the ESG framework on the ultra-high resolution datasets.}
%     \label{fig:gpu}
% \end{figure}

\qi{To address the aforementioned limitations, we present a novel model that can be adapted to both frameworks to cater for the different demand.} Specifically, our proposed model serves as the local segmentation module of CSM without introducing additional computational overhead for contexts beyond the local patch. Additionally, it can be directly used for the global inference of EGS, achieving better segmentation performance than prior art. To accomplish this, we drew inspiration from the idea of implicit neural representation (INR) \cite{chen2021learning} and designed an efficient spatial-guided high-resolution query module. This module enhances shallow-deep fusion in image detail inference, enabling our model to infer high-quality pixel-wise segmentation results. Our model queries the latent embeddings of the nearest spatial coordinates and the high-resolution spatial information as guidance, reducing the dependency on extra contextual information to the largest extent. Unlike previous feature fusion \cite{hu2022learning}, our approach guides the latent embeddings to supplement details through structurally interpretable shallow masks, which is more efficient and effective. However, the high-resolution spatial information tends to introduce semantic estimation bias during inference. To address this concern, we introduce a memory-based interaction scheme to bridge the semantic information of low-resolution features and high-resolution spatial information. This scheme implicitly introduces cross-image context for semantic-level regularization.




% In reality, considering different hardware conditions, an effective model capable of both local and global inference is essential. Thus, there is an intuitive attempt to study a context-weakening local function to efficiently segment objects/regions of different granularity in ultra-high resolution image. Inspired by xxx, we propose a novel "three-level implicit mask-guided function" to segment ultra-high resolution image, especially geospatial image captured from aerial views. Different from the previous model used upsampling and convolution that may blur the detailed information. In this function, the semantic information is represented by latent codes distributed in spatial dimensions. Only given a corresponding coordinate, it can independently output the precise result by querying the latent code closest to the coordinate and relative coordinate to the latent code. 

% Concretely, we perform the queries in two stages using three-level latent codes to prevent a large resolution gap. In both stages, the features at a deep semantic level are viewed as latent codes, and the remaining two levels use the mask as spatial guided latent codes. 

% Concretely, performing queries relying only on one-level semantic features as latent codes will still lack spatial details, we introduce a two-level mask with higher resolution to guide the query. However, due to the resolution gap, the semantic information is easily submerged by spatial masks. Thus, we propose a two-stage progressive query, the implicit function generates the higher resolution latent codes guided by the first-level mask, and then the final semantic result is output by the two-level mask in the second stage.
% But, the first-level mask tends to contain weak semantic information spatially, which may lead to undesired guidance. To this end, we design a "cross-level class memory module" that stores the semantic knowledge of each class from the semantic level. It dynamically updates the contents of memory under the supervision of the ground truth and invokes memory to weigh the first-level mask via the correlation between features. That is, this level is deemed as the guided-memory mixing level, acting on the "three-level implicit mask-guided function" collaborated with the semantic and remaining spatial levels.

% This function outputs the precise result by querying the corresponding coordinate in two stages. 

% In addition, ultra-high resolution image tends to cover many fine-grained objects/regions. The above models apply bilinear up-sampling or deconvolution at the decoding stage, which may blur the precise detail information and then lead to undesired results, especially for ultra-high resolution geospatial image captured from aerial views.

% To alleviate the aforementioned concerns, we propose a novel "two-stage implicit mask-guided function" that queries a single coordinate to obtain the corresponding segmentation result. It consists of just vanilla MLPs without much cost and achieves context-weakened dependence at the decoding stage.
% In concrete, features from deep network are viewed as latent codes, and masks from shallow network guide its detail in this function. And it takes as inputs the nearest latent code of the queried coordinate and the relative coordinates to the latent code to output the class of queried coordinate via two-stage. 
% Although the mask generated by shallow network has a lot of detailed information, its lack of semantics generates redundant noise which interferes with the query of coordinates. Thus, we design an effective "cross-network class memory module" that stores semantic information of features from deep network. It enhances the guide of the mask from shallow network only with simple steps when querying coordinates.

In comprehensive experiments for ultra-high resolution image segmentation task, we demonstrate that our proposed model can better trade off performance, memory, and efficiency in the both inference framework, and surpass the latest off-the-shelf methods on the DeepGlobe and Inria Aerial datasets. 

Overall, the main contributions of our paper are:
\begin{itemize}
    \item We propose the spatial-guided high-resolution query module based on a shallow-deep fusion network, which can be adapted to both CSM and EGS frameworks.
    \item In order to correct the semantic bias of spatial guidance, we present a memory-based interaction scheme to implicitly introduce cross-image context for high-resolution query.
%     \item We present a xxx function that utilizes mask-guided latent codes to query categories on image coordinates while also reducing context dependence.
%     \item To compensate for the semantics of shallow network masks, we introduce a xxx module to yield semantic memory of deep network features to enhance the guiding role of masks.
    \item Our model achieves the state-of-the-art semantic segmentation performance and accuracy-memory trade-off in the ultra-high resolution image datasets.
\end{itemize}


% 局部：显存低，速度慢，需要局部图像外的上下文(速度和显存)
% 全局：分辨率提高显存高，速度快，需要一些全局上下文
% 减弱上下文(局部的解码)，增强细节(插值)

==> a_intro_v2.tex <==
\section{Introduction}

\IEEEPARstart{W}{ith} the rapid progress of photography and sensor technologies, there is a growing demand for ultra-high resolution image (i.e., 2K, 4K, or even higher resolution images) analysis due to the unique role in remote sensing and medical applications, such as urban planning, environmental assessment, and medical diagnosis. However, handling ultra-high resolution image, especially for semantic segmentation task, will cost more unaffordable computing resources.

Recently, a promising solution has been proposed to address ultra-high resolution semantic segmentation using a shallow-deep fusion based global segmentation framework~\cite{guo2022isdnet}. This approach combines the high-resolution yet noisy semantic estimation from a shallow network with the low-resolution semantic estimation from a deep network, resulting in an efficient and effective solution. However, the fusion process also introduces noise and results in a loss of details. More importantly, as input image resolutions continue to increase, this method demands a substantially greater amount of GPU memory, rendering it impractical for systems with limited memory resources.
% memory is limited to less than 2GB due to hardware constraints.
Thus, is it possible to handle semantic segmentation of arbitrarily large images using limited memory? 

To resolve this problem, it is appropriate to resort to segmenting local patches instead of the entire ultra-high resolution image before merging all local segmentation results. However, this approach often leads to degraded performance, and thus additional context beyond the local patch needs to be introduced to address this concern in prior methods~\cite{chen2019collaborative, huynh2021progressive, li2021contexts}. Unfortunately, the introduction of additional context also results in increased memory usage.
In this paper, we propose a novel method for performing local segmentation without relying on context beyond local patches. This approach results in a memory-efficient and effective framework for ultra-high resolution semantic segmentation. 



% Rethinking the earlier cropping-segmenting-merging (CSM) framework \cite{chen2019collaborative, huynh2021progressive, li2021contexts}, local patch segmentation of ultra-high resolution image can reduce the demand for memory, but it will consume much time due to multiple local inference. Besides, extra context beyond the local patch needs to be introduced to avoid degraded local segmentation caused by too narrow a view, which also brings more memory usage and time consumption. To address the aforementioned limitations, we aim to design a novel model based on CSM framework that can also better trade off segmentation performance, memory usage, and computational overhead. 

In particular, we draw inspiration from the idea of implicit neural representation (INR)~\cite{chen2021learning} and design an efficient spatial-guided high-resolution query module,
% . This module enhances shallow-deep fusion in image detail inference, 
enabling our model to infer high-quality pixel-wise segmentation results. In specific, our model queries the nearest latent embeddings of the spatial coordinates and the high-resolution spatial information as guidance, reducing the dependency on extra contextual information beyond the local patch to the largest extent. 
% Unlike previous feature alignment~\cite{hu2022learning}, 
Moreover, we propose to guide the latent embeddings to supplement the details through high-resolution semantic masks in a more straightforward manner. However, the high-resolution spatial information tends to introduce semantic estimation bias during inference. \qi{To address this concern, we introduce a memory-based interaction scheme that efficiently facilitates the high-resolution semantics learning from compact cross-image contextual representation.
% bridge the semantic information of low-resolution features and high-resolution spatial information. 
% This scheme implicitly introduces cross-image context for semantic-level regularization.
Compared with previous memory-based schemes, our designed scheme adds up only 1MB GPU memory computational overhead thanks to its linear complexity.}

Through comprehensive experiments, we demonstrate that our proposed model can outperform the state-of-the-art approaches under the condition of limited memory over DeepGlobe and Inria Aerial datasets. Besides, our model also can better trade off segmentation performance, memory usage, and computational overhead than the latest off-the-shelf methods in unlimited memory systems.
% In addition, we also conduct experiments on the high-resolution CityScapes dataset to evaluate the generality for our model.

Overall, the main contributions of our paper are:
\begin{itemize}
    \item We propose a memory-efficient and effective model to handle semantic segmentation for an image with arbitrarily large resolution under a memory-limited condition.
    \item A novel spatial-guided high-resolution query module is introduced to predict semantic masks of local image patches without requiring additional contextual cues beyond the local region.
    \item We propose an efficient memory-based interaction scheme to address the issue of semantic bias arising from the local nature of image patches, which incorporates cross-image contextual information for high-resolution query, and introduces only a mild extra memory overhead. 
    \item Our model achieves superior performance in ultra-high resolution image segmentation, surpassing prior methods by a substantial margin, particularly under memory-limited conditions. Moreover, our approach offers a balanced trade-off between segmentation performance, memory usage, and computational overhead, in the absence of memory constraints.
\end{itemize}

==> figure/ifa.tex <==
\begin{figure}[t]
    \centering
    \footnotesize
	\begin{tabular}{c@{}c@{}c@{}c}

        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/ifa/321711_sat.jpg} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/ifa/321711_mask.png} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/ifa/ours_321711_sat.jpg} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/ifa/ifa_321711_sat.jpg} \\

        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/ifa/925382_sat.jpg} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/ifa/925382_mask.png} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/ifa/ours_925382_sat.jpg} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/ifa/ifa_925382_sat.jpg} \\
        
        Input Image & Ground-truth & Ours & IFA\cite{hu2022learning}
        
	\end{tabular}
	\caption{Examples show the efficacy of our spatial-guided high-resolution query compared with IFA\cite{hu2022learning}.}
	\label{fig:ifa}
\end{figure}

==> figure/mem.tex <==
\begin{figure}[t]
    \centering
    \footnotesize
	\begin{tabular}{c@{}c@{}c@{}c}

        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/mem/454655_sat.jpg} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/mem/454655_mask.png} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/mem/1ours_454655_sat.jpg} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/mem/1mem_454655_sat.jpg} \\

        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/mem/671164_sat.jpg} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/mem/671164_mask.png} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/mem/ours_671164_sat.jpg} &
        \includegraphics[width=0.12\textwidth,height=2.1cm]{figure/mem/mem_671164_sat.jpg} \\
        
        Input Image & Ground-truth & w Memory & w/o Memory
        
	\end{tabular}
	\caption{Examples show the efficacy of our memory-based interaction scheme.}
	\label{fig:mem}
\end{figure}

==> table/ab_less.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{12pt}
    \caption{The investigation for less memory usage.}
    \footnotesize
    \begin{tabular}{cccc}
        \toprule
        Dataset & mIoU & Memory & FPS \\
        \midrule
        DeepGlobe & 73.66 & 1472 & 10.09 \\
        DeepGlobe & 72.34 & 1036 & 4.68 \\ 
        Inria Aerial & 77.25 & 1324 & 3.55 \\
        Inria Aerial & 77.09 & 1036 & 1.83 \\
        \bottomrule
    \end{tabular}
    \label{tab:less}
\end{table}

==> table/com_IA.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{6pt}
    \caption{Comparison with state-of-the-arts on Inria Aerial.}
    \footnotesize
    \begin{tabular}{ccccc}
        \toprule      
        Model & Backbone & mIoU & Memory & FPS \\
        \midrule
        \multicolumn{5}{c}{\textit{\textbf{Memory is limited to 1.5GB}}} \\
        ISDNet* \cite{guo2022isdnet} & ResNet-18 & 74.74 & 1306 & 3.99 \\
        Ours & ResNet-18 & 77.25 & 1324 & 3.55 \\
        \midrule
        \multicolumn{5}{c}{\textit{\textbf{Memory is not limited to 1.5GB}}} \\
        FCN-8s \cite{long2015fully} & VGG-16 & 69.10 & 2447 & 1.90 \\
        DeepLab v3+ \cite{chen2018encoder} & ResNet-50 & 55.90 & 5122 & 1.67 \\
        STDC \cite{fan2021rethinking} & STDC & 72.44 & 7410 & 4.97 \\
        CascadePSP \cite{cheng2020cascadepsp} & ResNet-50 & 69.40 & 3236 & 0.03 \\
        GLNet \cite{chen2019collaborative} & ResNet-50 & 71.20 & 2663 & 0.05 \\
        FCtL \cite{li2021contexts} & VGG-16 & 72.87 & 4332 & 0.04 \\
        ISDNet \cite{guo2022isdnet} & ResNet-18 & 74.23 & 4680 & 6.90 \\
        Ours & ResNet-18 & 77.27 & 4834 & 5.53 \\
        \bottomrule
    \end{tabular}
    \label{tab:com_inria}
\end{table}
% \begin{table}
%     \centering
%     \setlength{\tabcolsep}{6pt}
%     \footnotesize
%     \begin{tabular}{ccccc}
%         \toprule      
%         \textit{CSM} & Backbone & mIOU & FPS & Memory  \\
%         \midrule
%         FCN-8s \cite{long2015fully} & VGG-16 & 69.10 & 1.90 & 2447 \\
%         DeepLab v3+ \cite{chen2018encoder} & ResNet-50 & 55.90 & 1.67 & 5122 \\
%         CascadePSP \cite{cheng2020cascadepsp} & ResNet-50 & 69.40 & 0.03 & 3236 \\
%         GLNet \cite{chen2019collaborative} & ResNet-50 & 71.20 & 0.05 & 2663 \\
%         FCtL \cite{li2021contexts} & VGG-16 & 72.87 & 0.04 & 4332 \\
%         ISDNet \cite{guo2022isdnet} & ResNet-18 & 74.74 & 3.99 & 1306 \\
%         Ours & ResNet-18 & 77.25 & - & - \\
%         \midrule
%         \textit{SDF} & Backbone & mIOU & FPS & Memory  \\
%         \midrule
%         STDC \cite{fan2021rethinking} & STDC & 72.44 & 4.97 & 7410 \\
%         ISDNet \cite{guo2022isdnet} & ResNet-18 & 74.23 & 6.90 & 4680 \\
%         Ours & ResNet-18 & 77.27 & - & - \\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison with state-of-the-arts on Inria Aerial.}
%     \label{tab:com_inria}
% \end{table}

==> table/com_deep.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{6pt}
    \caption{Comparison with state-of-the-arts on DeepGlobe. }
    \footnotesize
    \begin{tabular}{ccccc}
        \toprule
        Model & Backbone & mIoU & Memory & FPS \\
        \midrule
        \multicolumn{5}{c}{\textit{\textbf{Memory is limited to 1.5GB}}} \\
        % U-Net \cite{ronneberger2015u} & U-Net & 46.53 & 1741 & 1.26 \\
        FCN-8s \cite{long2015fully} & VGG-16 &  62.43 & 970 & 4.55 \\
        % DeepLab v3+ \cite{chen2018encoder} & ResNet-50 & 69.69 & 1541 & 1.60 \\      
        PPN \cite{wu2020patch} & ResNet-50 & 71.90 & 1193 & 12.90 \\
        ISDNet* \cite{guo2022isdnet} & ResNet-18 & 72.79 & 1440 & 11.47 \\
        Ours & ResNet-18 & 73.68 & 1472 & 10.09 \\
        \midrule
        \multicolumn{5}{c}{\textit{\textbf{Memory is not limited to 1.5GB}}} \\
        U-Net \cite{ronneberger2015u} & U-Net & 50.11 & 7627 & 3.54 \\
        FCN-8s \cite{long2015fully} & VGG-16 & 52.86 & 1984 & 7.91 \\
        DeepLab v3+ \cite{chen2018encoder} & ResNet-50 & 63.50 & 3226 & 4.44 \\
        BiSeNetV1 \cite{yu2018bisenet} & ResNet-18 & 53.00 & 1801 & 14.20 \\
        STDC  \cite{fan2021rethinking} & STDC & 70.30 & 2580 & 14.00 \\
        CascadePSP \cite{cheng2020cascadepsp} & ResNet-50 & 68.50 & 3236 & 0.11 \\
        GLNet \cite{chen2019collaborative} & ResNet-50 & 71.60 & 1865 & 0.17 \\
        PointRend \cite{kirillov2020pointrend} & HRNet & 71.78 & 1593 & 6.25 \\
        MagNet-Fast \cite{huynh2021progressive} & HRNetV2-W18  & 71.85 & 1559 & 3.40 \\
        MagNet \cite{huynh2021progressive} &  HRNetV2-W18 & 72.96 & 1559 & 0.80 \\
        FCtL \cite{li2021contexts} & VGG-16 & 72.76 & 4332 & 0.13 \\
        ISDNet \cite{guo2022isdnet} & ResNet-18 & 73.30 & 1948 & 27.70 \\
        Ours & ResNet-18 & 73.50 & 1966 & 24.33 \\
        Ours & ResNet-18 & 73.80 & 2378 & 15.22 \\
        \bottomrule
    \end{tabular}
    \label{tab:com_deepglobe}
\end{table}

% \begin{table}
%     \centering
%     \setlength{\tabcolsep}{6pt}
%     \footnotesize
%     \begin{tabular}{ccccc}
%         \toprule
%         \textit{CSM} & Backbone & mIoU & Memory & FPS \\
%         \midrule
%         U-Net \cite{ronneberger2015u} & U-Net & 46.53 & 1741 & 1.26 \\
%         FCN-8s \cite{long2015fully} & VGG-16 &  62.43 & 970 & 4.55 \\
%         DeepLab v3+ \cite{chen2018encoder} & ResNet-50 & 69.69 & 1541 & 1.60 \\
%         CascadePSP \cite{cheng2020cascadepsp} & ResNet-50 & 68.50 & 3236 & 0.11 \\
%         GLNet \cite{chen2019collaborative} & ResNet-50 & 71.60 & 1865 & 0.17 \\
%         PPN \cite{wu2020patch} & ResNet-50 & 71.90 & 1193 & 12.90 \\
%         MagNet-Fast \cite{huynh2021progressive} & HRNetV2-W18  & 71.85 & 1559 & 3.40 \\
%         MagNet \cite{huynh2021progressive} &  HRNetV2-W18 & 72.96 & 1559 & 0.80 \\
%         FCtL \cite{li2021contexts} & VGG-16 & 72.76 & 4332 & 0.13 \\
%         ISDNet \cite{guo2022isdnet} & ResNet-18 & 72.79 & 1440 & 11.47 \\
%         % Segformer \cite{xie2021segformer} & ? & ? & ? & ? \\
%         % UperNet \cite{xiao2018unified} & ? & ? & ? & ? \\
%         Ours & ResNet-18 & 73.68 & 1472 & 10.09 \\
%         \midrule
%         \textit{SDF} & Backbone & mIoU & Memory & FPS \\
%         \midrule
%         U-Net \cite{ronneberger2015u} & U-Net & 50.11 & 7627 & 3.54 \\
%         FCN-8s \cite{long2015fully} & VGG-16 & 52.86 & 1984 & 7.91 \\
%         DeepLab v3+ \cite{chen2018encoder} & ResNet-50 & 63.50 & 3226 & 4.44 \\
%         BiSeNetV1 \cite{yu2018bisenet} & ResNet-18 & 53.00 & 1801 & 14.20 \\
%         STDC  \cite{fan2021rethinking} & STDC & 70.30 & 2580 & 14.00 \\
%         PointRend \cite{kirillov2020pointrend} & HRNet & 71.78 & 1593 & 6.25 \\
%         ISDNet \cite{guo2022isdnet} & ResNet-18 & 73.30 & 1948 & 27.70 \\
%         Ours & ResNet-18 & 73.50 & 1966 & 24.33 \\
%         Ours & ResNet-18 & 73.80 & 2378 & 15.22 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison with state-of-the-arts on DeepGlobe. }
%     \label{tab:com_deepglobe}
% \end{table}

% \begin{table}
%     \centering
%     \setlength{\tabcolsep}{6pt}
%     \footnotesize
%     \begin{tabular}{ccccc}
%         \toprule
%         \textit{CSM} & Backbone & mIOU & FPS & Memory  \\
%         \midrule
%         U-Net \cite{ronneberger2015u} & U-Net & 46.53 & 1.26 & 1741 \\
%         FCN-8s \cite{long2015fully} & VGG-16 &  62.43 & 4.55 & 970 \\
%         DeepLab v3+ \cite{chen2018encoder} & ResNet-50 & 69.69 & 1.60 & 1541 \\
%         CascadePSP \cite{cheng2020cascadepsp} & ResNet-50 & 68.50 & 0.11 & 3236 \\
%         GLNet \cite{chen2019collaborative} & ResNet-50 & 71.60 & 0.17 & 1865 \\
%         PPN \cite{wu2020patch} & ResNet-50 & 71.90 & 12.90 & 1193 \\
%         MagNet-Fast \cite{huynh2021progressive} & HRNetV2-W18  & 71.85 & 3.40 & 1559 \\
%         MagNet \cite{huynh2021progressive} &  HRNetV2-W18 & 72.96 & 0.80 & 1559 \\
%         FCtL \cite{li2021contexts} & VGG-16 & 72.76 & 0.13 & 4332 \\
%         ISDNet \cite{guo2022isdnet} & ResNet-18 & 72.79 & - & - \\
%         Ours & ResNet-18 & 73.68 & - & - \\
%         \midrule
%         \textit{SDF} & Backbone & mIOU & FPS & Memory \\
%         \midrule
%         U-Net \cite{ronneberger2015u} & U-Net & 50.11 & 3.54 & 7627 \\
%         FCN-8s \cite{long2015fully} & VGG-16 & 52.86 & 7.91 & 1984 \\
%         DeepLab v3+ \cite{chen2018encoder} & ResNet-50 & 63.50 & 4.44 & 3226 \\
%         BiSeNetV1 \cite{yu2018bisenet} & ResNet-18 & 53.00 & 14.20 & 1801 \\
%         STDC  \cite{fan2021rethinking} & STDC & 70.30 & 14.00 & 2580 \\
%         PointRend \cite{kirillov2020pointrend} & ResNet-50 & 71.78 & 6.25 & 1593 \\
%         ISDNet \cite{guo2022isdnet} & ResNet-18 & 73.30 & 27.70 & 1948 \\
%         Ours & ResNet-18 & 73.80 & - & - \\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison with state-of-the-arts on DeepGlobe. }
%     \label{tab:com_deepglobe}
% \end{table}
